Space observations of AA Doradus provide consistent mass determinations. New HW-Vir systems observed with TESS

We present an overview of eclipsing systems of the HW-Virginis type, based on space observations from the TESS Mission. We perform a detailed analysis of the properties of AA Dor, which was monitored for almost a full year. This excellent time-series dataset permitted us to search for both stellar pulsations and eclipse timing variations. In addition, we used the high-precision trigonometric parallax from Gaia Early Data Release 3 to make an independent determination of the fundamental stellar parameters. No convincing pulsations were detected down to a limit of 76 parts per million, however we detected one peak with false alarm probability of 0.2%. 20 sec cadences being collected during Year 3 should confirm or reject our detection. From eclipse timing measurements we were able to confirm that the orbital period is stable, with an upper limit to any period change of 5.75 $\cdot$ 10$^{-13}$ s/s. The apparent offset of the secondary eclipse is consistent with the predicted R{\o}mer delay when the primary mass is that of a canonical extended horizontal branch star. Using parallax and a spectral energy distribution corroborates that the mass of the primary in AA Dor is canonical, and its radius and luminosity is consistent with an evolutionary state beyond core helium burning. The mass of the secondary is found to be at the limit of hydrogen burning.

==> LB3459_photometry_results_bb.tex <==
%\documentclass{standalone}
%%\usepackage{amsmath,txfonts,color}
%\usepackage[colorlinks=true,urlcolor=black]{hyperref}
%\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lr}
\hline\hline
%Object: LB3459 & 68\% confidence interval\\
%\hline
%Color excess $E(B-V)$ from \href{https://ui.adsabs.harvard.edu/abs/1998ApJ...500..525S/abstract}{SFD (1998)} & $0.69\pm0.17$\,mag \\
%Color excess $E(B-V)$ from \href{https://ui.adsabs.harvard.edu/abs/2011ApJ...737..103S/abstract}{S\&F (2011)} & $0.59\pm0.15$\,mag \\
%\hline
Color excess $E(B-V)$ & $0.014^{+0.022}_{-0.014}$\,mag \\
%Extinction parameter $R(55)$ (fixed) & $3.02$ \\
Angular diameter $\log(\Theta\,\mathrm{(rad)})$ & $-10.600^{+0.029}_{-0.038}$ \\
%Parallax $\varpi$ ({\it Gaia}, $\text{RUWE}=0.98$, $\text{offset}=0.029\,\text{mas}$) & $2.75\pm0.06$\,mas \\
%Effective temperature $T_{\mathrm{eff}}$ (prescribed) & $42000\pm1000$\,K \\
%Surface gravity $\log (g\,\mathrm{(cm\,s^{-2})})$ (prescribed) & $5.46\pm0.05$ \\
%Microturbulence $\xi$ (fixed) & $0$\,km\,s$^{-1}$ \\
%Metallicity $z$ (fixed) & $0$\,dex \\
%Helium abundance $\log(n(\textnormal{He}))$ (fixed) & $-3.16$ \\
Radius $R = \Theta/(2\varpi)$ & $0.204^{+0.014}_{-0.019}$\,$R_\odot$ \\
Mass $M = g R^2/G$ & $0.42\pm0.09$\,$M_\odot$ \\
Luminosity $L/L_\odot = (R/R_\odot)^2(T_\mathrm{eff}/T_{\mathrm{eff},\odot})^4$ & $112^{+22}_{-21}$ \\
%Gravitational redshift $\varv_\mathrm{grav} = GM/(Rc)$ & $1.32^{+0.21}_{-0.18}$\,km\,s${}^{-1}$ \\
\hline
\multicolumn{2}{l}{Blackbody component:} \\
Blackbody temperature $T_{\mathrm{bb}}$ & $12000^{+\phantom{0}6000}_{-11900}$\,K \\
Blackbody surface ratio $A_\mathrm{eff,bb}/A_{\mathrm{eff}}$ & $0.48^{+0.37}_{-0.24}$ \\
\hline
Generic excess noise $\delta_\textnormal{excess}$ & $0.018$\,mag \\
%Reduced $\chi^2$ at the best fit & $1.00$ \\
%Parameter reference & 2011A\&A...531L...7K \\
\hline
\end{tabular}
%\end{document}


==> LB3459_photometry_results_bin.tex <==
%\documentclass{standalone}
%\usepackage{amsmath,txfonts,color}
%\usepackage[colorlinks=true,urlcolor=black]{hyperref}
%\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lr}
\hline\hline
%Object: LB3459 & 68\% confidence interval\\
%\hline
%Color excess $E(B-V)$ from \href{https://ui.adsabs.harvard.edu/abs/1998ApJ...500..525S/abstract}{SFD (1998)} & $0.69\pm0.17$\,mag \\
%Color excess $E(B-V)$ from \href{https://ui.adsabs.harvard.edu/abs/2011ApJ...737..103S/abstract}{S\&F (2011)} & $0.59\pm0.15$\,mag \\
%\hline
Color excess $E(B-V)$ & $0.007^{+0.012}_{-0.007}$\,mag \\
%Extinction parameter $R(55)$ (fixed) & $3.02$ \\
Angular diameter $\log(\Theta\,\mathrm{(rad)})$ & $-10.610^{+0.018}_{-0.020}$ \\
%Parallax $\varpi$ ({\it Gaia}, $\text{RUWE}=0.98$, $\text{offset}=0.029\,\text{mas}$) & $2.75\pm0.06$\,mas \\
\hline
\multicolumn{2}{l}{Component 1:} \\
%Effective temperature $T_{\mathrm{eff}}$ (prescribed) & $42000\pm1000$\,K \\
%Surface gravity $\log (g\,\mathrm{(cm\,s^{-2})})$ (prescribed) & $5.46\pm0.05$ \\
%Microturbulence $\xi$ (fixed) & $0$\,km\,s$^{-1}$ \\
%Metallicity $z$ (fixed) & $0$\,dex \\
%Helium abundance $\log(n(\textnormal{He}))$ (fixed) & $-3.16$ \\
Radius $R = \Theta/(2\varpi)$ & $0.198\pm0.010$\,$R_\odot$ \\
Mass $M = g R^2/G$ & $0.41^{+0.07}_{-0.06}$\,$M_\odot$ \\
Luminosity $L/L_\odot = (R/R_\odot)^2(T_\mathrm{eff}/T_{\mathrm{eff},\odot})^4$ & $108^{+16}_{-14}$ \\
%Gravitational redshift $\varv_\mathrm{grav} = GM/(Rc)$ & $1.30^{+0.18}_{-0.16}$\,km\,s${}^{-1}$ \\
\hline
\multicolumn{2}{l}{Component 2:} \\
Effective temperature $T_{\mathrm{eff}}$ & $10700^{+3600}_{-1600}$\,K \\
%Surface gravity $\log (g\,\mathrm{(cm\,s^{-2})})$ (prescribed) & $4.0\pm0.5$ \\
%Microturbulence $\xi$ (fixed) & $0$\,km\,s$^{-1}$ \\
%Metallicity $z$ (fixed) & $0$\,dex \\
%Helium abundance $\log(n(\textnormal{He}))$ (fixed) & $-1.05$ \\
Surface ratio $A_\mathrm{eff}/A_{\mathrm{eff,}1}$ & $1.0\pm0.4$ \\
Radius $R = (A_\mathrm{eff}/A_{\mathrm{eff,}1})^{1/2}\Theta/(2\varpi)$ & $0.20^{+0.04}_{-0.05}$\,$R_\odot$ \\
%Mass $M = g R^2/G$ & $0.0028^{+0.0203}_{-0.0026}$\,$M_\odot$ \\
Luminosity $L/L_\odot = (R/R_\odot)^2(T_\mathrm{eff}/T_{\mathrm{eff},\odot})^4$ & $0.23^{+0.54}_{-0.19}$ \\
%Gravitational redshift $\varv_\mathrm{grav} = GM/(Rc)$ & $0.011^{+0.065}_{-0.010}$\,km\,s${}^{-1}$ \\
\hline
Generic excess noise $\delta_\textnormal{excess}$ & $0.014$\,mag \\
%Reduced $\chi^2$ at the best fit & $1.00$ \\
%Parameter reference & 2011A\&A...531L...7K \\
\hline
\end{tabular}
%\end{document}


==> LB3459_photometry_results_single.tex <==
%\documentclass{standalone}
%\usepackage{amsmath,txfonts,color}
%\usepackage[colorlinks=true,urlcolor=black]{hyperref}
%\begin{document}
%\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lr}
\hline\hline
%Object: LB3459 & 68\% confidence interval\\
%\hline
%Color excess $E(B-V)$ from \href{https://ui.adsabs.harvard.edu/abs/1998ApJ...500..525S/abstract}{SFD (1998)} & $0.69\pm0.17$\,mag \\
%Color excess $E(B-V)$ from \href{https://ui.adsabs.harvard.edu/abs/2011ApJ...737..103S/abstract}{S\&F (2011)} & $0.59\pm0.15$\,mag \\
%\hline
Color excess $E(B-V)$ & $0.035\pm0.005$\,mag \\
%Extinction parameter $R(55)$ (fixed) & $3.02$ \\
Angular diameter $\log(\Theta\,\mathrm{(rad)})$ & $-10.571\pm0.007$ \\
%Parallax $\varpi$ ({\it Gaia}, $\text{RUWE}=0.98$, $\text{offset}=0.029\,\text{mas}$) & $2.75\pm0.06$\,mas \\
%Effective temperature $T_{\mathrm{eff}}$ (prescribed) & $42000\pm1000$\,K \\
%Surface gravity $\log (g\,\mathrm{(cm\,s^{-2})})$ (prescribed) & $5.46\pm0.05$ \\
%Microturbulence $\xi$ (fixed) & $0$\,km\,s$^{-1}$ \\
%Metallicity $z$ (fixed) & $0$\,dex \\
%Helium abundance $\log(n(\textnormal{He}))$ (fixed) & $-3.16$ \\
Radius $R = \Theta/(2\varpi)$ & $0.216\pm0.006$\,$R_\odot$ \\
Mass $M = g R^2/G$ & $0.49^{+0.07}_{-0.06}$\,$M_\odot$ \\
Luminosity $L/L_\odot = (R/R_\odot)^2(T_\mathrm{eff}/T_{\mathrm{eff},\odot})^4$ & $130^{+15}_{-14}$ \\
%Gravitational redshift $\varv_\mathrm{grav} = GM/(Rc)$ & $1.43^{+0.19}_{-0.16}$\,km\,s${}^{-1}$ \\
\hline
Generic excess noise $\delta_\textnormal{excess}$ & $0.020$\,mag \\
%Reduced $\chi^2$ at the best fit & $1.00$ \\
%Parameter reference & 2011A\&A...531L...7K \\
\hline
\end{tabular}
%\end{document}

